AdamP: Slowing Down the Slowdown for Momentum Optimizers on Scale-invariant Weights

Normalization techniques are a boon for modern deep learning. They let weights converge more quickly with often better generalization performances. It has been argued that the normalization-induced scale invariance among the weights provides an advantageous ground for gradient descent (GD) optimizers: the effective step sizes are automatically reduced over time, stabilizing the overall training procedure. It is often overlooked, however, that the additional introduction of momentum in GD optimizers results in a far more rapid reduction in effective step sizes for scale-invariant weights, a phenomenon that has not yet been studied and may have caused unwanted side effects in the current practice. This is a crucial issue because arguably the vast majority of modern deep neural networks consist of (1) momentum-based GD (e.g. SGD or Adam) and (2) scale-invariant parameters. In this paper, we verify that the widely-adopted combination of the two ingredients lead to the premature decay of effective step sizes and sub-optimal model performances. We propose a simple and effective remedy, SGDP and AdamP: get rid of the radial component, or the norm-increasing direction, at each optimizer step. Because of the scale invariance, this modification only alters the effective step sizes without changing the effective update directions, thus enjoying the original convergence properties of GD optimizers. Given the ubiquity of momentum GD and scale invariance in machine learning, we have evaluated our methods against the baselines on 13 benchmarks. They range from vision tasks like classification (e.g. ImageNet), retrieval (e.g. CUB and SOP), and detection (e.g. COCO) to language modelling (e.g. WikiText) and audio classification (e.g. DCASE) tasks. We verify that our solution brings about uniform gains in those benchmarks. Source code is available at https://github.com/clovaai/AdamP.

==> 4.Experiments.old.tex <==
\definecolor{darkergreen}{RGB}{21, 152, 56}
\newcommand\greenp[1]{\textcolor{darkergreen}{(#1)}}
\definecolor{red2}{RGB}{252, 54, 65}
\newcommand\redp[1]{\textcolor{red2}{(#1)}}
\newcommand\greenpscript[1]{\scriptsize\greenp{#1}}
\newcommand\redpscript[1]{\scriptsize\redp{#1}}

\section{Experiments}
\label{sec:experiments}

In this section, we demonstrate the effectiveness of our projection module for training scale-invariant weights with momentum-based optimizers. We experiment over various real-world tasks and datasets. From the image domain, we show results on ImageNet classification~(\S\ref{sec:exp-imgclassification}), object detection~(\S\ref{sec:exp-imgdetection}), and robustness benchmarks~(\S\ref{sec:exp-advtr}). From the audio domain, we study music tagging, speech recognition, and sound event detection~(\S\ref{sec:exp-audio}).
Finally, the metric learning experiments with $\ell_2$ normalized embeddings~(\S\ref{sec:exp-retrieval}) show that our method works also on the scale invariances that do not originate from the statistical normalization.
In the above set of experiments, we show that the proposed modifications (\sgdn and \adamn) bring consistent performance gains against the baselines (SGD~\citep{nag} and Adam~\citep{adam}).
We provide the implementation details in the Appendix~\ref{appendixsec:settings}.

\subsection{Image classification}
\label{sec:exp-imgclassification}

Batch normalization (BN) and momentum-based optimizer are standard techniques to train state-of-the-art image classification models~\citep{resnet,pyramidnet,mobilenetv2}.
We evaluate the proposed method with ResNet~\citep{resnet}, one of the most popular and powerful architectures on ImageNet, and MobileNetV2~\citep{mobilenetv2}, a relatively lightweight model with ReLU6 and depthwise convolutions, on the ImageNet-1K benchmark~\citep{imagenet}. For ResNet, we employ the training hyperparameters in \citep{resnet}. For MobileNetV2, we have searched for the best setting, as it is generally difficult to train it with the usual settings. We use the cosine annealed learning rates for all experiments.

Our optimizers \sgdn and \adamn are compared against their corresponding baselines in Table~\ref{table:classification}. Across the spectrum of network sizes from MobileNetV2 to ResNet50, our optimizers outperform the baselines. Even when the state-of-the-art CutMix~\citep{cutmix} regularization is applied, our optimizers bring further gains.

\begin{table}[h]
\centering
\small
\vspace{-.5em}
\caption{\small \textbf{ImageNet classification.} Accuracies of state-of-the-art networks trained with \sgdn and \adamn.}
\label{table:classification}
\vspace{.0em}
\begin{tabular}{@{}llccccc@{}}
\toprule
Architecture                  & \# params & SGD & \sgdn (ours) & Adam & AdamW & \adamn (ours)\\ \midrule
MobileNetV2 &  3.5M     & 71.61 & \textbf{72.18 \greenpscript{+0.57}}  & 69.27  & 72.12 & \textbf{72.57 \greenpscript{+0.45}} \\ 
ResNet18 &  11.7M    & 70.28 & \textbf{70.73 \greenpscript{+0.45}}  & 68.05  & 70.41 & \textbf{70.81 \greenpscript{+0.40}} \\ 
ResNet50 &  25.6M    & 76.64 & \textbf{76.71 \greenpscript{+0.07}}  & 71.89  & 76.65 & \textbf{76.94 \greenpscript{+0.29}} \\
ResNet50 + CutMix &  25.6M    & 77.61 & \textbf{77.72 \greenpscript{+0.11}}  & 76.41  & 78.00 & \textbf{78.31 \greenpscript{+0.31}} \\ \bottomrule
\end{tabular}
\vspace{-.5em}
\end{table}

\begin{wraptable}{r}{0.4\linewidth}
\setlength{\tabcolsep}{3.5pt}
\vspace{-1.7em}
\small
\centering
\caption{\small\textbf{Weight decay.} Optimizer performances for training ResNet18 on ImageNet.}
\label{table:cls_wd}
\vspace{.5em}
\begin{tabular}{@{}lcc@{}}
\toprule
              & Baseline & w/o weight decay \\ \midrule
SGD           & 70.28    & 67.94 \redpscript{-2.38}  \\
\sgdn (ours)  & 70.73    & 70.21 \redpscript{-0.52}  \\
AdamW          & 70.41    & 68.52 \redpscript{-1.89}  \\ 
\adamn (ours) & 70.81    & 70.50 \redpscript{-0.31}   \\ \bottomrule
\end{tabular}
\end{wraptable}

\paragraph{Impact of weight decay.}
Projection is not the only way to suppress the norm increases. Weight decay (WD) is another simple way to regularize them. Note that WD is used throughout our experiments.
We study the effects of removing WD for each optimizer considered.
Table~\ref{table:cls_wd} shows the results. Removing WD results in performance drops, signifying the importance of the weight norm regularization. For \sgdn and \adamn, however, the drops are less dramatic. As our optimizers already regularize the norm growth, the models rely less on WD for suppressing the norms. Our method thus lifts the burden for practitioners to choose WD carefully. We report the weight norms and effective step sizes for various WD values in the Appendix~\ref{appendixsec:lr_and_wd}.

\subsection{Robustness}
\label{sec:exp-advtr}

Model robustness is an emerging problem in real-world applications of machine learning. Due to the inherent difficulty of the problem, methods typically involve complex optimization problems. We examine how our optimizers stabilize the complex optimization problems.

\begin{wrapfigure}{r}{0.41\linewidth}
    \vspace{-1.6em}
    \includegraphics[width=\linewidth]{figures/l2_adv.pdf}
    \includegraphics[width=\linewidth]{figures/linf_adv.pdf}
    \vspace{-2em}
    \caption{\small \textbf{Adversarial training.} Learning curves by Adam and \adamn.}
    \vspace{-2em}
    \label{fig:advtr_adam_vs_adamn}
\end{wrapfigure}

\paragraph{Adversarial robustness.}
Adversarial training alternatively optimizes a minimax problem where the inner optimization is an adversarial attack and the outer optimization is the standard classification problem. Adam is commonly used for the adversarial training in order to handle the complexity of the optimization.
The adversarial robustness remains a difficult problem; even the current best solutions have large generalization gaps between the standard accuracies and attacked accuracies~\citep{tsipras2018robustness,chun2019icmlw}.

In our experiments, we train Wide-ResNet~\citep{wideresnet} with the projected gradient descent (PGD)~\citep{madry2018towards} attacks. We use 10 inner PGD iterations and $\varepsilon=80/255$ for the $L_2$ PGD attack and $\varepsilon=4/255$ for the $L_\infty$ PGD attack.
Figure~\ref{fig:advtr_adam_vs_adamn} shows the effect of \adamn. 
By handling the effective step sizes, \adamn achieves a faster convergence than Adam (less than half the epochs required); loss plots in the Appendix. \adamn brings more than $+9.3$ pp performance gap in all settings.

\paragraph{Robustness against real-world biases.}
Cross-bias generalization problem~\citep{bahng2019rebias} tackles the scenario where the training and test distributions have different real-world biases. This often occurs when the training-set biases provide an easy shortcut to solve the problem: \eg, using the snow cues for recognizing snowmobiles. \citep{bahng2019rebias} has proposed the ReBias scheme based on the minimax optimization, where the inner problem maximizes the independence between an intentionally biased representation and the target model of interest and the outer optimization solves the standard classification problem. As for the adversarial training, \citep{bahng2019rebias} has employed the Adam to handle the complex optimization. 

We follow the two cross-bias generalization benchmarks proposed by \citep{bahng2019rebias}. The first benchmark is the Biased MNIST, the dataset synthesized by injecting colors on the MNIST background pixels. Each sample is colored according to a pre-defined class-color mapping with probability $\rho$. The color is selected at random with $1-\rho$ chance. For example, $\rho=1.0$ leads a completely biased dataset and $\rho=0.1$ leads to an unbiased dataset. Each model is trained on the $\rho$-biased MNIST and tested on the unbiased MNIST. We train a stacked convolutional network with BN and ReLU. 
The second benchmark is the 9-Class ImageNet representing the real-world biases, such as textures~\citep{stylised_imagenet}. The unbiased accuracy is measured by pseudo-labels generated by the texture clustering. We also report the performance on ImageNet-A~\citep{imagenet_a}, the collection of failure samples of existing CNNs.

In Table~\ref{tab:rebias}, we observe that \adamn consistently outperforms Adam in all the benchmarks. AdamP is a good alternative to Adam for difficult optimization problems applied on scale-invariant parameters.

\begin{table}[ht!]
\setlength{\tabcolsep}{3.5pt}
\centering
\caption{\small \textbf{Real-world bias robustness.} Biased MNIST and 9-Class ImageNet benchmarks with ReBias~\citep{bahng2019rebias}.}
\label{tab:rebias}
\vspace{0em}
\small
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multirow{2}{*}{Optimizer} & \multicolumn{5}{c}{Biased MNIST Unbiased acc. at $\rho$} & & \multicolumn{3}{c}{9-Class ImageNet} \\ \cmidrule(l){2-6} \cmidrule(l){8-10}
      & .999 & .997 & .995 & .990 & avg. & & Biased     & UnBiased     & ImageNet-A     \\ \midrule
Adam  & 22.9           & 63.0           & 74.9           & 87.0       & 61.9          & & 93.8      & 92.6        & 31.2    \\
\adamn (ours) & \textbf{30.5 \greenpscript{+7.5}}           & \textbf{70.9 \greenpscript{+7.9}}           & \textbf{80.9 \greenpscript{+6.0}}           & \textbf{89.6 \greenpscript{+2.6}}  & \textbf{68.0 \greenpscript{+6.0}}    &      & \textbf{95.2 \greenpscript{+1.4}}      & \textbf{94.5 \greenpscript{+1.8}}        & \textbf{32.9 \greenpscript{+1.7}}    \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Audio classification}
\label{sec:exp-audio}

We evaluate the proposed optimizer on three different audio classification tasks with different physical properties: music clips, verbal audios, and acoustic signals.
For automatic music tagging, we use the MagnaTagATune (MTAT) benchmark~\citep{mtat} with 21k samples and 50 tags. Each clip contains multiple tags.
We also use the Speech Commands dataset~\citep{speechcommands} for the keyword spotting task (106k samples, 35 classes, one-hot label).
For acoustic signals, we use the sound event detection dataset from the DCASE 2017 challenge~\citep{dcase} (53k samples, 17 tags), where each audio has multiple tags.

We trained the Harmonic CNN~\citep{won2020harmonic} on the three benchmarks. Harmonic CNN consists of data-driven harmonic filters, stacked convolutional filters with BN.
Audio datasets are usually smaller than the image datasets and are multi-labeled, posing another set of difficulty for the optimization problem.
\citep{won2020harmonic} has employed the mixed optimizer with Adam and SGD proposed by \citep{won2019attention}.
Instead of the mixture solution, we have searched the best hyperparameters for the Adam baseline and our \adamn on a validation set.
The results are given in Table~\ref{table:audio}. \adamn shows better performance than the baselines, without having to adopt the complex mixture of Adam and SGD. The audio experiments signify the superiority of \adamn for training scale-invariant weights on a non-image domain.

\begin{table}[ht!]
\centering
\small
\vspace{0em}
\caption{\small \textbf{Audio classification.} Results on three audio classification tasks with Harmonic CNN~\citep{won2020harmonic}. }
\label{table:audio}
\vspace{0em}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{Optimizer} & \multicolumn{2}{c}{Music Tagging}    & Keyword Spotting & Sound Event Tagging \\ \cmidrule(l){2-5} 
& ROC-AUC       & PR-AUC                & Accuracy         & F1 score \\ \midrule
Adam + SGD~\citep{won2019attention} & 91.27 & 45.67 & 96.08 & 54.60 \\
Adam & 91.12 & 45.61 & 96.47 & 55.24 \\
\adamn (ours) & \textbf{91.35 \greenp{+0.23}} & \textbf{45.79 \greenp{+0.18}} & \textbf{96.89 \greenp{+0.42}} & \textbf{56.04 \greenp{+0.80}} \\ \bottomrule
\end{tabular}
\vspace{-.5em}
\end{table}

\subsection{Language modeling}
\begin{wraptable}{r}{0.47\linewidth}
\setlength{\tabcolsep}{4pt}
\centering
\small
\vspace{-2em}
\caption{\small\textbf{Language Modeling.} Perplexity of Transformer-XL~\citep{dai2019transformer} trained with Adam and \adamn optimizers on WikiText-103.}
\label{table:language}
\begin{tabular}{@{}lcc@{}}
\toprule
Model        & Adam   & \adamn (ours)  \\ \midrule
Transformer-XL & 23.33  & \textbf{23.26 \greenpscript{-0.07}} \\
Transformer-XL + WN  & 23.90  & \textbf{22.73 \greenpscript{-1.17}} \\
\bottomrule
\end{tabular}
\vspace{-0em}
\end{wraptable}

\ho{
To explore the impact of the proposed \adamn~optimizer on language modeling, we use Transformer-XL~\citep{dai2019transformer} to WikiText-103~\citep{merity2016pointer}, a word-level language modeling benchmark.
In the Transformer architecture \citep{vaswani2017attention}, there is a residual connection between a fully-connected layer and a normalization layer which makes the parameters not scale-invariant even with the normalization layer.
Therefore, there is no significant performance gain of \adamn over Adam in Transformer-XL, as shown in the first row of Table~\ref{table:language}.
To make the parameters scale-invariant, we apply weight normalization (WN) \citep{weightnorm} to all of the linear layers in the Transformer-XL.
The result is shown in the second row of Table~\ref{table:language}.
When trained with Adam optimizer, WN decreases the performance, but if trained with \adamn, WN improves the model's performance.
This result implies that \adamn can contribute to models with few scale-invariant parameters through weight normalization, and the effect of weight normalization should be re-measured considering \adamn.
}
